Introduction to Presentation Attack Detection in Fingerprint Biometrics

This chapter provides an introduction to Presentation Attack Detection (PAD) in fingerprint biometrics, also coined anti-spoofing, describes early developments in this field, and briefly summarizes recent trends and open issues.

==> Makefile <==
# Created by Sebastien Marcel <marcel@idiap.ch> 
# Wed 12 Apr 15:18:46 CEST 2017

# Builds the LaTeX project as a PDF document

TEXFILE=author.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex 
	latex $(@:%.pdf=%.tex)
	makeindex -s svind.ist author.idx
	makeindex -t author.glg -o author.gls -s myglo.ist author.glo
	@if [ -e references.bib ]; then \
	 bibtex $(@:%.pdf=%); \
	 latex $(@:%.pdf=%); \
	fi
	latex $(@:%.pdf=%.tex)
	dvipdf author

all: $(PDFFILE)

.PHONY: clean 

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.gls *.glg *.dvi *.ps *.pdf *.out *.brf

